Fairness Uncertainty Quantification: How certain are you that the model is fair?

Fairness-aware machine learning has garnered significant attention in recent years because of extensive use of machine learning in sensitive applications like judiciary systems. Various heuristics, and optimization frameworks have been proposed to enforce fairness in classification \cite{del2020review} where the later approaches either provides empirical results or provides fairness guarantee for the exact minimizer of the objective function \cite{celis2019classification}. In modern machine learning, Stochastic Gradient Descent (SGD) type algorithms are almost always used as training algorithms implying that the learned model, and consequently, its fairness properties are random. Hence, especially for crucial applications, it is imperative to construct Confidence Interval (CI) for the fairness of the learned model. In this work we provide CI for test unfairness when a group-fairness-aware, specifically, Disparate Impact (DI), and Disparate Mistreatment (DM) aware linear binary classifier is trained using online SGD-type algorithms. We show that asymptotically a Central Limit Theorem holds for the estimated model parameter of both DI and DM-aware models. We provide online multiplier bootstrap method to estimate the asymptotic covariance to construct online CI. To do so, we extend the known theoretical guarantees shown on the consistency of the online bootstrap method for unconstrained SGD to constrained optimization which could be of independent interest. We illustrate our results on synthetic and real datasets.

==> Uncertainty Quantification of Fairness-aware Models_arxiv/rebuttal.tex <==
\textbf{Reviewer fp72}
Thank you for your valuable comments.

Weaknesses:

    ``The paper assumes that the main source of estimation uncertainty of the fairness metric lies in stochasticity of the training algorithm ... stochastic training of model parameters might be relatively small compared to, say, bias in training data distribution":
    
    We want to clarify here that we do not * assume * the main source to be stochasticity of the training algorithm. As we have mentioned, and shown through experiment, in the Introduction (line 29-62), that stochasticity of the training algorithm can be a significant source of randomness in the fairness. Our goal is to characterize and quantify this randomness. Notice that the ** source of the stochasticity in the algorithm is indeed the training data distribution and that does get captured through Theorem 4.1, and Theorem 4.2 specifically through $\Sigma_{DI(DM)}$. Theoretical guarantees on estimation of this randomness is in Theorem 5.1. ** 
    
     
Questions:

    ``What is significance or interpretation of the convergence result in Theorem 5.1 3? We care about the error between the estimated DI using bootstrap vs the true DI under the optimal parameter . The bound suggests that the difference between either of the term and behaves similarly, but what does it imply about the behavior of the error as iterations gets large?"

    Theorem 5.1 (3) shows that the ** distribution of the bootstrap estimator converges to the true distribution of the algorithmic estimator of fairness as the iterations grow large. Note that behavior of the error between the algorithmic estimator $bar{\theta}_n$ and the true parameter $\theta^*$ when the iteration gets large is captured in Theorem 4.1 and 4.2. But we want to emphasize here that we are not only trying to minimize this error; rather we are addressing a more challenging problem where we characterize and estimate the distribution of this error in order to form confidence interval for the fairness. So showing convergence of error to 0 is not enough. Since we have only one trajectory and one $\bar{\theta}_n$ after training stops, we need to * estimate * the distribution of $\bar{\theta}_n$ in order to construct confidence interval for $\phi_{DI}(\theta^*)$. The bootstrap process is proposed to estimate the asymptotic distribution of $\phi_{DI}(\bar{\theta}_n)$ obtained in Theorem 4.1 and 4.2. Theorem 5.1 provides theoretical guarantees with $1/\sqrt{n}$ rate that the distribution approximated using these bootstrap samples $\hat{\phi}_{DI}\{\bar{\theta}_n^b\}$ indeed converges to the distribution of $\phi_{DI}\bar{\theta}_n$ which in turns provides theoretical validity of the constructed confidence intervals.** 


    Figure 1 shows that DI is unstable in different iterations of the training process, especially in the early stage of training. This is an interesting experimental result. Since we are not optimizing for small DI/DM but rather optimizing accuracy subject to DI/DM constraint, does DI/DM stabilizes once the constraint is satisfied?

    We respectfully disagree with the interpretation of Figure 1. Please have a look at the bottom left figure in Figure 1 where we magnify the green region of the top left figure. It shows that ** towards the end of training, while all the trajectories and consequently, the mean DI level (blue line) is almost constant, different runs of the training algorithm with the same initial point can produce widely varying DI levels. We are indeed optimizing for accuracy (equation (4) and (6)) with the constraints enforcing DI and DM to be small. But unlike canonical studies, instead of looking at the uncertainties in accuracy, we study the randomness in the fairness of the model. Figure 1 is there as the motivation of studying this problem showing that even if the individual training trajectories, and the mean level of DI and DM has stabilized, there can be considerable randomness due to the stochasticity of the training algorithm. **

    We can do a bootstrap method on testing set using trained model to get a confidence interval on the fairness metric directly. What is the advantage of considering the online estimation problem given that we care more about the fairness metrics of the model after it is trained?

    Bootstrapping after training, that is keeping the trained model fixed, only captures the randomness in the test data. Since models are trained using stochastic optimization method, the ** trained model itself is random. Online covariance estimation is required to capture the randomness due to the stochasticity in the training dynamics which inherently induces a Markov chain. ** 

    **Fairness uncertainty quantification is certainly an important topic and one would imagine its estimation error would also be related to other factors such as the bias in training and testing datasets in addition to stochasticity in training. Could you discuss how this work fit in the broader picture?**

We agree that it would be indeed interesting to explicitly study the relation between uncertainties present in fairness and bias/imbalance in the training and test data. We would like to mention that we do characterize the uncertainties due to the stochasticity of training procedure/algorithm which essentially originates from the training data. So the asymptotic covariance $\Sigma_{DI}$, and $\Sigma_{DI}$, and the confidence interval constructed does capture the effect of the training data distribution on uncertainty. 

Please reach out to us in the discussion phase if there are additional questions and we will be happy to provide the required clarification. 

\textbf{Reviewer DCkP}

Thank you for your valuable comments.

WRITING CLARITY. Thank you for such a thorough review. We will correct these errors and clarify the writing. We do agree that the text is missing quite a few necessary explanatory details due to space constraint. If it gets accepted, we promise to do a much better job since we will have one more page to explain properly in the camera-ready version. 


``Does this work only categorize the fairness constraints as constructed in Zafar et al, i.e., using the convex proxy function they use for the DI-aware model?"

In short yes. To elaborate, if the problem is non-convex then there can be multiple global minima, saddle points and local minima. In this case, a result like Theorem 4.1, and 4.2 becomes meaningless since there is no particular $\theta^*$ the algorithm is converging to. Results on uncertainty quantification with theoretical guarantee is broadly missing for general stochastic nonconvex optimization.

``If the penalty is constructed in a different way does that change the theoretical results?"

The theoretical results will hold as long as Assumptions 4.1 - 4.6 hold. Any change in penalty will be captured by the $P_A$ matrix in Theorem 4.1 and $R_2^2\nabla \gamma(\theta;{\mathcal{D}'}^{-}\nabla \gamma(\theta;{{\mathcal{D}'}^{-}}^\top)$ in Theorem 4.2. 

``Does the penalized version of the problem introduced by Zafar that the authors consider for DM change the quality of the models returned by the learner?"

They perform pretty similar to the one presented in Zafar et. al. For example, in Figure 5 for the COMPAS dataset,  Zafar et. al. reports a DM(FPR) of 0.03 whereas ours is 0.05. Notice that, similar to covariance threshold $c$ in Zafar et. al.'s paper, $R_2$ is the tuning parameter in Algorithm 2 in this paper. To achieve a lower fairness guarantee we need to increasing $R_2$. We did not include a comparison of the performance of our algorithm and Zafar et. al.'s work since our goal was not to propose a better fairness-ensuring model compared to Zafar et. al; rather we wanted to quantify the randomness present in a fairness-aware stochastic algorithm. If accepted, we will include the results on comparison of the two approaches in the final draft. 

\textbf{Reviewer Erji}
Thank you for your valuable comments.

``The two measures of algorithmic fairness presented in section 3 are widely known in the literature. I would not include them as proper definitions of the paper. Moreover, I find convenient mentioning that each of them is measuring a different fairness criteria: DI measures Demographic Parity, while DM quantifies Equality of Odds."

We agree. We will remove it from the final draft and this will also give us space to explain the work in more detail. 


``In section 4, the fulfilment of some of the hypotheses is discussed very briefly, but a discussion of 4.4 and 4.5 is missing."

Thanks for pointing this out. There is actually a typo in Assumption 4.4. It should actually be $\|\nabla l(\theta)\|_2^2\leq C(1+\|\theta\|_2^2)$. This implies that the norm of the gradient of the loss function $\nabla l(\theta)$ grows at most linearly with the norm of $\theta$. This holds true for all commonly used loss functions like squared loss, Huber loss, cross-entropy loss, and smoothed Hinge loss. 

Assumption 4.5 implies that the covariance of the random variable $\nabla L(\theta^*,W_k)$ holds asymptotically. In other words, the tail of the random variable should be such that at least the variance exists. This is a required assumption for any asymptotic normality result since without this assumption the normality is not even well defined. 

We will explain this in the final draft. 
    
``Page 2 (top), the reference to the figure is missing."

We will fix it. 
    
``In Theorem 4.1. some notations are not clear. Questions:
    Is it possible an extension of similar results to the regression framework?"

It is indeed possible to extend this to regression framework. For example see reference [1] below. In fact, as shown in [1], fair regression can be reduced to a constrained classification problem and similar guarantees may be provided. This is indeed quite an interesting idea. 

[1] Agarwal, Alekh, Miroslav Dudík, and Zhiwei Steven Wu. "Fair regression: Quantitative definitions and reduction-based algorithms." In International Conference on Machine Learning, pp. 120-129. PMLR, 2019.

\textbf{Reviewer E7Th}

Thank you for your valuable comments.


``The setting of online learning of a fair classifier does not appear organically. I think the theoretical results for the SDA procedure for online learning of an empirical risk minimizer can stand on its own, with fairness being a toy illustrative example. I say toy because the datasets considered here do not arise in an online fashion at all....Finally a compelling example of an online fair classification task should be included. "

We chose these datasets since ** these are two of the most widely-known datasets used to illustrate these group fairness metrics only in offline but for online fairness-aware classification. For a non-exhaustive list of works using these datasets for online fair classification please see [3,4,5,6,7,8] below. ** If you could elaborate on what you mean by ``data appearing in online fashion organically" we hope to answer this question better.

``Also the strongly-convex requirement on the loss function severely limits the algorithmic fairness applications that can be dealt with.....The strongly-convex requirement precludes many commonly used classifiers in modern settings. "

Since this is the first work on UQ of fairness, we limited ourselves to strongly convex loss. But we emphasize that this assumption holds for all linear classification set up including logistic regression, and SVM for logistic and squared loss. It even holds for ultra-wide Neural Networks (See reference [1] below). We do agree that extensions to general and more realistic neural network setting will be more challenging and really interesting as we mention in the Future work. In fact for general neural network setting, since the loss landscape is nonconvex, a CLT type result may not be well-defined (also see our reply to Reviewer DCkP). 

``The bootstrap is extremely expensive and ... "

The bootstrap procedure at most changes the gradient computation by $O(1)$ since $B$ is constant and does not grow with iteration $n$. These bootstrap sample computations can be parallelized easily since they do not affect each other.  Additionally, the bootstrap does not impose any extra data-burden since all the bootstrap samples are evaluated using the same data-point. 

``...it is unclear if the computational burden is justified (do we really need those CIs in the early iterations?)"

This is an excellent idea and we expect that practically it can improve the performance considerably. To establish the theoretical guarantees on almost sure and distributional convergence (Theorem 5.1), one needs to compute the bootstrap samples for at least the tail of the Markov chain that is induced by the optimization. 

`` It also seems strange to me that we receive training data in a sequential manner but we assume there is a fairly large, fixed, held-out dataset available to us to form the CIs."

Online training is often preferred even if the whole dataset is available due to computational cost of treating huge datasets at once. So we decouple the training dynamics, which actually involves the heavy computation, from the computationally cheap final phase of the fairness inference which essentially involves evaluation of dot products of two vectors only. This held-out dataset can interpreted as the first few observations which is not used in the training phase. This concept has been used for online inference in other contexts as well [9-11]. 

``I think it would also be helpful to discuss whether the costly bootstrap is really worth the extra computation."

We are using bootstrap to approximate the distribution of $\bar{\theta}_n$. If we remove the bootstrap procedure then we just have one sample $\bar{\theta}_n$ and one cannot construct a CI anymore. 


``I would like to understand better why we need online UQ for group fairness? It would be great to see a motivating application. The datasets analyzed in the experiment (compas and adult) are far from this online setting."

As we have mentioned above these are two of the most widely-used datasets for ** online fair classification ** See [3-8] below. 

[1] Liu, Chaoyue, Libin Zhu, and Misha Belkin. "On the linearity of large non-linear models: when and why the tangent kernel is constant." Advances in Neural Information Processing Systems 33 (2020): 15954-15964.

[2]Anastasiou, Andreas, Krishnakumar Balasubramanian, and Murat A. Erdogdu. "Normal approximation for stochastic gradient descent via non-asymptotic rates of martingale CLT." In Conference on Learning Theory, pp. 115-137. PMLR, 2019.

[3] Iosifidis, Vasileios, Wenbin Zhang, and Eirini Ntoutsi. "Online fairness-aware learning with imbalanced data streams." arXiv preprint arXiv:2108.06231 (2021).

[4] Aguiar, Gabriel, Bartosz Krawczyk, and Alberto Cano. "A survey on learning from imbalanced data streams: taxonomy, challenges, empirical study, and reproducible experimental framework." arXiv preprint arXiv:2204.03719 (2022).

[5] Iosifidis, Vasileios, Thi Ngoc Han Tran, and Eirini Ntoutsi. "Fairness-enhancing interventions in stream classification." In Database and Expert Systems Applications: 30th International Conference, DEXA 2019, Linz, Austria, August 26–29, 2019, Proceedings, Part I 30, pp. 261-276. Springer International Publishing, 2019.

[6] Sun, Yi, Ivan Ramirez, Alfredo Cuesta-Infante, and Kalyan Veeramachaneni. "Learning fair classifiers in online stochastic settings." CoRR, abs/1908.07009 (2019).

[7] Zhang, Wenbin, and Liang Zhao. "Online decision trees with fairness." arXiv preprint arXiv:2010.08146 (2020).

[8] Zhao, Chen, Feng Chen, and Bhavani Thuraisingham. "Fairness-aware online meta-learning." In Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery & Data Mining, pp. 2294-2304. 2021.

[9] Canini, Kevin, Lei Shi, and Thomas Griffiths. "Online inference of topics with latent Dirichlet allocation." In Artificial Intelligence and Statistics, pp. 65-72. PMLR, 2009.

[10] Gupta, Chirag, Aleksandr Podkopaev, and Aaditya Ramdas. "Distribution-free binary classification: prediction sets, confidence intervals and calibration." Advances in Neural Information Processing Systems 33 (2020): 3711-3723.

[11] Xu, Chen, and Yao Xie. "Conformal prediction set for time-series." arXiv preprint arXiv:2206.07851 (2022).

[12] Chai, Junyi, and Xiaoqian Wang. "Fairness with adaptive weights." In International Conference on Machine Learning, pp. 2853-2866. PMLR, 2022.

[13] Guardieiro, Vitória, Marcos M. Raimundo, and Jorge Poco. "Enforcing fairness using ensemble of diverse Pareto-optimal models." Data Mining and Knowledge Discovery (2023): 1-29.

[14] Kamp, Serafina, Andong Luis Li Zhao, and Sindhu Kutty. "Robustness of Fairness: An Experimental Analysis." In Machine Learning and Principles and Practice of Knowledge Discovery in Databases: International Workshops of ECML PKDD 2021, Virtual Event, September 13-17, 2021, Proceedings, Part I, pp. 591-606. Cham: Springer International Publishing, 2022.

[15] Zhang, Yiliang, and Qi Long. "Assessing fairness in the presence of missing data." Advances in neural information processing systems 34 (2021): 16007-16019.

[16] Scutari, Marco, Francesca Panero, and Manuel Proissl. "Achieving fairness with a simple ridge penalty." Statistics and Computing 32, no. 5 (2022): 77.



``The properties of SDA estimator for constrained DI is studied in Section 4.1 while the properties of vanilla SGD with averaging is studied for the constrained DM problem in Section 4.2. I'm a bit confused about Section 4.2. Isn't this already covered in Fang et al 2018?"

This has been covered much before Fang et al 2018 in Polyak and Juditsky 1992 as we have stated after Theorem 4.2. Since the goal of our paper is to perform uncertainty quantification for fairness, and not proving a CLT for SGD iterates, we included this result for completion as Disparate Mistreatment is one of the most widely used fairness measures. 

``I was confused by the notation in Section 4.1. are the sensitive attributes in the training data . However are also referred to as the sequence of updates which is a weighted sum of all noisy gradients up to time . Have you perhaps double-loaded the notation for ?"

We have indeed double-loaded the notation. We will fix it in the final version. 

``Shouldn't the convergence in distribution result in Thm 4.1 be in terms of rather than ?"

We have used $n$ instead of $k$ to denote that $\bar{\theta}_n$ is the final iterate of the algorithm. But we understand why it could be confusing. We will change the notation. 

``

It seems like SDA is used to solve the constrained DI problem (Eqn 5), but vanilla SGD with Polyak-Ruppert averageing is used to solve the penalized DM problem (Eqn 7). Hasn't Fang et al already provided the theoretical results for UQ of vanilla SGD with PR averaging? Your contribution is geared towards SDA if I understand correctly. Is it necessary to spend time in this paper on the latter challenge if it's already more-or-less solved using Fang's results?"

This is true and we have clearly stated it in lines 322-327 that we extend the results of Fang et. al. 2018 to the SDA setting. Also we have mentioned after Theorem 4.2 that the results follow from  Polyak \& Juditsky, 1992. The only reason we have included this section is that, our goal is to do uncertainty quantification for fairness. Disparate Mistreatment (DM) is one of the most widely used fairness metric. For the sake of completion, we presented these results which hold for the alternative modeling of DM we propose. We will try to emphasize it more that the main theoretical contribution of this paper is towards SDA.

Dear PC, Senior AC and AC, 

We have several concerns about the reviews which we have elaborated. 

In summary, 

a) we urge you to consider that irrespective of the scores, all the **reviewers acknowledge that this is the first work** on Uncertainty Quantification (UQ) of fairness where we propose **a practically implementable algorithm with theoretical guarantee and illustrate its results on state-of-the-art classifiers and benchmark datasets**. 

b) We feel the scores are unfair since the reviewers consider **Theorem 5.1 as groundbreaking (Reviewer DCkP) and that it can stand on its own (Reviewer E7Th), but recommend "Reject" due to grammatical errors (Reviewer DCkP), misunderstanding of the results (Reviewer fp72), or because they felt that benchmark datasets ( Reviewer Erji agrees with us) in online fairness classification literature are just ``toy" examples (Reviewer E7Th).**

We would appreciate if you could take this into consideration and at least ignore the review of Reviewer fp72 or find another expert reviewer to evaluate the contributions of our paper. Thanks a lot for your consideration.

Sincerely

Authors






**Detailed concerns**

1. It appears to us that Reviewer fp72 is truly unaware of stochastic optimization and distributional convergence. They correctly identify that Theorem 5.1 is the main theoretical contribution but by their own admission in Q1, Reviewer fp72 does not understand what Theorem 5.1 says (which is distributional convergence of bootstrap estimator).  

2. Reviewer fp72 claims (Q2) "Figure 1 shows that DI is unstable ... especially in the early stage" whereas Fig. 1 shows the exact opposite that towards the end stage, when the trajectory is stable, there can be significant variations due to the stochasticity of the algorithm.

3. Reviewer fp72 claims that (Q3) ``can do a bootstrap method on testing set using trained model to get a confidence interval" which completely misses the fact that the trained model itself is random and the bootstrap method is designed to capture that.

4. Reviewer fp72 claims (Q4) that the stochasticity of the algorithm does not capture the effect of training distribution whereas the only source of randomness of the training algorithm is indeed the training data distribution and our results do capture that through the asymptotic covariance term.

5. The main criticism of Reviewer DCkP is that the paper has grammatical issues. 

6. Reviewer E7Th claims that state-of-the-art datasets used in online fairness-aware classification literature are toy examples and not organically online. Please find supporting citations in our reply to Reviewer E7Th.

Second reply to Reviewer E7Th.

"If we wanted to understand the variability in the fairness metric (DI/DM) arising from the stochasticity of the training dynamics, we simply need to repeat the training many times and record the resulting DI from each repetition. This seems more straightforward and vastly preferable to the proposed bootstrap procedure. ...."

We respectfully disagree on two accounts. 

a) Repeating the whole training many times with different training data **directly contradicts with online** training regime. In fact, the **main challenge** of online training is that the learner has access to **only one data point at every time step**, that is the we are **constructing the confidence interval** from a **single trajectory of data samples.**

b) Even if one relaxes online requirement, this approach still increases the data burden /sample complexity of the algorithms. 

We request you to kindly have a look at the inference results in online stochastic approximation literature [1-3] below. 

My bigger concern is ... For UQ to be useful in the setting you consider, we must understand how (classification loss, DI/DM) varies jointly in the accuracy-fairness space. It is not meaningful to consider only the fairness variability when the classification loss is also subject to the same forces of variability.

Note that our method and results characterize and estimate the uncertainty of the *model parameter* of a fairness-aware classification model. Since accuracy and fairness both depend on the same model parameter, using the same methods as in Algorithm 2 and Theorem 5.1, it is straightforward to get a similar result for accuracy as well. Indeed one can establish similar inference results for loss of a classifier as well. Since UQ of the fairness is the main gap in the research we are addressing here, we decided against providing a version of Theorem 5.1 for all possible properties of the classifier. In other words, **instead of looking at the joint distribution of accuracy/loss and fairness, we construct the confidence interval for the marginal distribution of fairness once the accuracy has stabilized. This is analogous to inference results for Gaussian mean estimation where the confidence intervals are constructed for the mean and not for other properties of the distribution, e.g., higher-order moments, skewness, kurtosis etc, even though the mean parameter of the Gaussian distribution controls all the properties of the distribution.**

[1] Polyak, Boris T., and Anatoli B. Juditsky. "Acceleration of stochastic approximation by averaging." SIAM journal on control and optimization 30, no. 4 (1992): 838-855.

[2] Duchi, John, and Feng Ruan. "Asymptotic optimality in stochastic optimization." arXiv preprint arXiv:1612.05612 (2016).

[3] Yixin Fang, Jinfeng Xu, and Lei Yang. Online bootstrap confidence intervals for the stochastic
gradient descent estimator. The Journal of Machine Learning Research, 19(1):3053–3073, 2018.



Dear AC, Senior AC, and PC, 

From response in the discussion period, it seems Reviewer E7Th is hostile and lacks understanding of the problem setting.

The first comment, "...we simply need to repeat the training many times..." clearly shows that Reviewer E7Th does not have the basic understanding of the online learning and stochastic approximation literature since the **main challenge** of inference of online stochastic approximation is to construct CI from a **single trajectory of data sequence with access to only one data point at each time point.** 

In the second comment, Reviewer E7Th claims that CI for fairness is meaningless without CI for loss/accuracy of the classifier since both depend on the variability in the model parameter. By this argument, for any inference to be meaningful, one needs to construct simultaneous CI for all possible properties of the model since all these properties depend on the variability of the estimated model parameter which is an absurd claim. For analogy, in Gaussian mean estimation, the confidence intervals are constructed for the mean and not for other properties of the distribution, e.g., higher-order moments, skewness, kurtosis etc, even though the mean parameter of the Gaussian distribution controls all the properties of the distribution.

We emphasize that our method and results characterize and estimate the uncertainty of the **model parameter of a fairness-aware classification model** and provide UQ of fairness when the training accuracy has reached a stable level. Since **UQ of the fairness is the main gap** in the research we are addressing here, we decided against providing a version of Theorem 5.1 for loss/accuracy of the classifier.  

We expect a fair review and request you to interfere. 

With regards,

Authors

Dear AC, Senior AC, and PC, 

 We draw your attention to the fact that **Reviewer fp72 has acknowledged that they initially misunderstood the paper and now has adjusted the score to 6.** This further strengthens our claim that **Reviewer E7Th is either hostile or has misunderstood the paper since they say their "initial hesitation towards this work is summed up by Reviewer fp72's Question 3".**

Furthermore, **Reviewer DCkP** has not got back to us with any further question. Reviewer DCkP's main criticism is that the paper has **grammatical/writing issues which is easily fixable.** We will do a thorough correction of these mistakes in the final version.

We request you to kindly take these into consideration.


With regards,
Authors



==> rebuttal.tex <==
\textbf{Reviewer fp72}
Thank you for your valuable comments.

Weaknesses:

    ``The paper assumes that the main source of estimation uncertainty of the fairness metric lies in stochasticity of the training algorithm ... stochastic training of model parameters might be relatively small compared to, say, bias in training data distribution":
    
    We want to clarify here that we do not * assume * the main source to be stochasticity of the training algorithm. As we have mentioned, and shown through experiment, in the Introduction (line 29-62), that stochasticity of the training algorithm can be a significant source of randomness in the fairness. Our goal is to characterize and quantify this randomness. Notice that the ** source of the stochasticity in the algorithm is indeed the training data distribution and that does get captured through Theorem 4.1, and Theorem 4.2 specifically through $\Sigma_{DI(DM)}$. Theoretical guarantees on estimation of this randomness is in Theorem 5.1. ** 
    
     
Questions:

    ``What is significance or interpretation of the convergence result in Theorem 5.1 3? We care about the error between the estimated DI using bootstrap vs the true DI under the optimal parameter . The bound suggests that the difference between either of the term and behaves similarly, but what does it imply about the behavior of the error as iterations gets large?"

    Theorem 5.1 (3) shows that the ** distribution of the bootstrap estimator converges to the true distribution of the algorithmic estimator of fairness as the iterations grow large. Note that behavior of the error between the algorithmic estimator $bar{\theta}_n$ and the true parameter $\theta^*$ when the iteration gets large is captured in Theorem 4.1 and 4.2. But we want to emphasize here that we are not only trying to minimize this error; rather we are addressing a more challenging problem where we characterize and estimate the distribution of this error in order to form confidence interval for the fairness. So showing convergence of error to 0 is not enough. Since we have only one trajectory and one $\bar{\theta}_n$ after training stops, we need to * estimate * the distribution of $\bar{\theta}_n$ in order to construct confidence interval for $\phi_{DI}(\theta^*)$. The bootstrap process is proposed to estimate the asymptotic distribution of $\phi_{DI}(\bar{\theta}_n)$ obtained in Theorem 4.1 and 4.2. Theorem 5.1 provides theoretical guarantees with $1/\sqrt{n}$ rate that the distribution approximated using these bootstrap samples $\hat{\phi}_{DI}\{\bar{\theta}_n^b\}$ indeed converges to the distribution of $\phi_{DI}\bar{\theta}_n$ which in turns provides theoretical validity of the constructed confidence intervals.** 


    Figure 1 shows that DI is unstable in different iterations of the training process, especially in the early stage of training. This is an interesting experimental result. Since we are not optimizing for small DI/DM but rather optimizing accuracy subject to DI/DM constraint, does DI/DM stabilizes once the constraint is satisfied?

    We respectfully disagree with the interpretation of Figure 1. Please have a look at the bottom left figure in Figure 1 where we magnify the green region of the top left figure. It shows that ** towards the end of training, while all the trajectories and consequently, the mean DI level (blue line) is almost constant, different runs of the training algorithm with the same initial point can produce widely varying DI levels. We are indeed optimizing for accuracy (equation (4) and (6)) with the constraints enforcing DI and DM to be small. But unlike canonical studies, instead of looking at the uncertainties in accuracy, we study the randomness in the fairness of the model. Figure 1 is there as the motivation of studying this problem showing that even if the individual training trajectories, and the mean level of DI and DM has stabilized, there can be considerable randomness due to the stochasticity of the training algorithm. **

    We can do a bootstrap method on testing set using trained model to get a confidence interval on the fairness metric directly. What is the advantage of considering the online estimation problem given that we care more about the fairness metrics of the model after it is trained?

    Bootstrapping after training, that is keeping the trained model fixed, only captures the randomness in the test data. Since models are trained using stochastic optimization method, the ** trained model itself is random. Online covariance estimation is required to capture the randomness due to the stochasticity in the training dynamics which inherently induces a Markov chain. ** 

    **Fairness uncertainty quantification is certainly an important topic and one would imagine its estimation error would also be related to other factors such as the bias in training and testing datasets in addition to stochasticity in training. Could you discuss how this work fit in the broader picture?**

We agree that it would be indeed interesting to explicitly study the relation between uncertainties present in fairness and bias/imbalance in the training and test data. We would like to mention that we do characterize the uncertainties due to the stochasticity of training procedure/algorithm which essentially originates from the training data. So the asymptotic covariance $\Sigma_{DI}$, and $\Sigma_{DI}$, and the confidence interval constructed does capture the effect of the training data distribution on uncertainty. 

Please reach out to us in the discussion phase if there are additional questions and we will be happy to provide the required clarification. 

\textbf{Reviewer DCkP}

Thank you for your valuable comments.

WRITING CLARITY. Thank you for such a thorough review. We will correct these errors and clarify the writing. We do agree that the text is missing quite a few necessary explanatory details due to space constraint. If it gets accepted, we promise to do a much better job since we will have one more page to explain properly in the camera-ready version. 


``Does this work only categorize the fairness constraints as constructed in Zafar et al, i.e., using the convex proxy function they use for the DI-aware model?"

In short yes. To elaborate, if the problem is non-convex then there can be multiple global minima, saddle points and local minima. In this case, a result like Theorem 4.1, and 4.2 becomes meaningless since there is no particular $\theta^*$ the algorithm is converging to. Results on uncertainty quantification with theoretical guarantee is broadly missing for general stochastic nonconvex optimization.

``If the penalty is constructed in a different way does that change the theoretical results?"

The theoretical results will hold as long as Assumptions 4.1 - 4.6 hold. Any change in penalty will be captured by the $P_A$ matrix in Theorem 4.1 and $R_2^2\nabla \gamma(\theta;{\mathcal{D}'}^{-}\nabla \gamma(\theta;{{\mathcal{D}'}^{-}}^\top)$ in Theorem 4.2. 

``Does the penalized version of the problem introduced by Zafar that the authors consider for DM change the quality of the models returned by the learner?"

They perform pretty similar to the one presented in Zafar et. al. For example, in Figure 5 for the COMPAS dataset,  Zafar et. al. reports a DM(FPR) of 0.03 whereas ours is 0.05. Notice that, similar to covariance threshold $c$ in Zafar et. al.'s paper, $R_2$ is the tuning parameter in Algorithm 2 in this paper. To achieve a lower fairness guarantee we need to increasing $R_2$. We did not include a comparison of the performance of our algorithm and Zafar et. al.'s work since our goal was not to propose a better fairness-ensuring model compared to Zafar et. al; rather we wanted to quantify the randomness present in a fairness-aware stochastic algorithm. If accepted, we will include the results on comparison of the two approaches in the final draft. 

\textbf{Reviewer Erji}
Thank you for your valuable comments.

``The two measures of algorithmic fairness presented in section 3 are widely known in the literature. I would not include them as proper definitions of the paper. Moreover, I find convenient mentioning that each of them is measuring a different fairness criteria: DI measures Demographic Parity, while DM quantifies Equality of Odds."

We agree. We will remove it from the final draft and this will also give us space to explain the work in more detail. 


``In section 4, the fulfilment of some of the hypotheses is discussed very briefly, but a discussion of 4.4 and 4.5 is missing."

Thanks for pointing this out. There is actually a typo in Assumption 4.4. It should actually be $\|\nabla l(\theta)\|_2^2\leq C(1+\|\theta\|_2^2)$. This implies that the norm of the gradient of the loss function $\nabla l(\theta)$ grows at most linearly with the norm of $\theta$. This holds true for all commonly used loss functions like squared loss, Huber loss, cross-entropy loss, and smoothed Hinge loss. 

Assumption 4.5 implies that the covariance of the random variable $\nabla L(\theta^*,W_k)$ holds asymptotically. In other words, the tail of the random variable should be such that at least the variance exists. This is a required assumption for any asymptotic normality result since without this assumption the normality is not even well defined. 

We will explain this in the final draft. 
    
``Page 2 (top), the reference to the figure is missing."

We will fix it. 
    
``In Theorem 4.1. some notations are not clear. Questions:
    Is it possible an extension of similar results to the regression framework?"

It is indeed possible to extend this to regression framework. For example see reference [1] below. In fact, as shown in [1], fair regression can be reduced to a constrained classification problem and similar guarantees may be provided. This is indeed quite an interesting idea. 

[1] Agarwal, Alekh, Miroslav Dudík, and Zhiwei Steven Wu. "Fair regression: Quantitative definitions and reduction-based algorithms." In International Conference on Machine Learning, pp. 120-129. PMLR, 2019.

\textbf{Reviewer E7Th}

Thank you for your valuable comments.


``The setting of online learning of a fair classifier does not appear organically. I think the theoretical results for the SDA procedure for online learning of an empirical risk minimizer can stand on its own, with fairness being a toy illustrative example. I say toy because the datasets considered here do not arise in an online fashion at all....Finally a compelling example of an online fair classification task should be included. "

We chose these datasets since ** these are two of the most widely-known datasets used to illustrate these group fairness metrics only in offline but for online fairness-aware classification. For a non-exhaustive list of works using these datasets for online fair classification please see [3,4,5,6,7,8] below. ** If you could elaborate on what you mean by ``data appearing in online fashion organically" we hope to answer this question better.

``Also the strongly-convex requirement on the loss function severely limits the algorithmic fairness applications that can be dealt with.....The strongly-convex requirement precludes many commonly used classifiers in modern settings. "

Since this is the first work on UQ of fairness, we limited ourselves to strongly convex loss. But we emphasize that this assumption holds for all linear classification set up including logistic regression, and SVM for logistic and squared loss. It even holds for ultra-wide Neural Networks (See reference [1] below). We do agree that extensions to general and more realistic neural network setting will be more challenging and really interesting as we mention in the Future work. In fact for general neural network setting, since the loss landscape is nonconvex, a CLT type result may not be well-defined (also see our reply to Reviewer DCkP). 

``The bootstrap is extremely expensive and ... "

The bootstrap procedure at most changes the gradient computation by $O(1)$ since $B$ is constant and does not grow with iteration $n$. These bootstrap sample computations can be parallelized easily since they do not affect each other.  Additionally, the bootstrap does not impose any extra data-burden since all the bootstrap samples are evaluated using the same data-point. 

``...it is unclear if the computational burden is justified (do we really need those CIs in the early iterations?)"

This is an excellent idea and we expect that practically it can improve the performance considerably. To establish the theoretical guarantees on almost sure and distributional convergence (Theorem 5.1), one needs to compute the bootstrap samples for at least the tail of the Markov chain that is induced by the optimization. 

`` It also seems strange to me that we receive training data in a sequential manner but we assume there is a fairly large, fixed, held-out dataset available to us to form the CIs."

Online training is often preferred even if the whole dataset is available due to computational cost of treating huge datasets at once. So we decouple the training dynamics, which actually involves the heavy computation, from the computationally cheap final phase of the fairness inference which essentially involves evaluation of dot products of two vectors only. This held-out dataset can interpreted as the first few observations which is not used in the training phase. This concept has been used for online inference in other contexts as well [9-11]. 

``I think it would also be helpful to discuss whether the costly bootstrap is really worth the extra computation."

We are using bootstrap to approximate the distribution of $\bar{\theta}_n$. If we remove the bootstrap procedure then we just have one sample $\bar{\theta}_n$ and one cannot construct a CI anymore. 


``I would like to understand better why we need online UQ for group fairness? It would be great to see a motivating application. The datasets analyzed in the experiment (compas and adult) are far from this online setting."

As we have mentioned above these are two of the most widely-used datasets for ** online fair classification ** See [3-8] below. 

[1] Liu, Chaoyue, Libin Zhu, and Misha Belkin. "On the linearity of large non-linear models: when and why the tangent kernel is constant." Advances in Neural Information Processing Systems 33 (2020): 15954-15964.

[2]Anastasiou, Andreas, Krishnakumar Balasubramanian, and Murat A. Erdogdu. "Normal approximation for stochastic gradient descent via non-asymptotic rates of martingale CLT." In Conference on Learning Theory, pp. 115-137. PMLR, 2019.

[3] Iosifidis, Vasileios, Wenbin Zhang, and Eirini Ntoutsi. "Online fairness-aware learning with imbalanced data streams." arXiv preprint arXiv:2108.06231 (2021).

[4] Aguiar, Gabriel, Bartosz Krawczyk, and Alberto Cano. "A survey on learning from imbalanced data streams: taxonomy, challenges, empirical study, and reproducible experimental framework." arXiv preprint arXiv:2204.03719 (2022).

[5] Iosifidis, Vasileios, Thi Ngoc Han Tran, and Eirini Ntoutsi. "Fairness-enhancing interventions in stream classification." In Database and Expert Systems Applications: 30th International Conference, DEXA 2019, Linz, Austria, August 26–29, 2019, Proceedings, Part I 30, pp. 261-276. Springer International Publishing, 2019.

[6] Sun, Yi, Ivan Ramirez, Alfredo Cuesta-Infante, and Kalyan Veeramachaneni. "Learning fair classifiers in online stochastic settings." CoRR, abs/1908.07009 (2019).

[7] Zhang, Wenbin, and Liang Zhao. "Online decision trees with fairness." arXiv preprint arXiv:2010.08146 (2020).

[8] Zhao, Chen, Feng Chen, and Bhavani Thuraisingham. "Fairness-aware online meta-learning." In Proceedings of the 27th ACM SIGKDD Conference on Knowledge Discovery & Data Mining, pp. 2294-2304. 2021.

[9] Canini, Kevin, Lei Shi, and Thomas Griffiths. "Online inference of topics with latent Dirichlet allocation." In Artificial Intelligence and Statistics, pp. 65-72. PMLR, 2009.

[10] Gupta, Chirag, Aleksandr Podkopaev, and Aaditya Ramdas. "Distribution-free binary classification: prediction sets, confidence intervals and calibration." Advances in Neural Information Processing Systems 33 (2020): 3711-3723.

[11] Xu, Chen, and Yao Xie. "Conformal prediction set for time-series." arXiv preprint arXiv:2206.07851 (2022).

[12] Chai, Junyi, and Xiaoqian Wang. "Fairness with adaptive weights." In International Conference on Machine Learning, pp. 2853-2866. PMLR, 2022.

[13] Guardieiro, Vitória, Marcos M. Raimundo, and Jorge Poco. "Enforcing fairness using ensemble of diverse Pareto-optimal models." Data Mining and Knowledge Discovery (2023): 1-29.

[14] Kamp, Serafina, Andong Luis Li Zhao, and Sindhu Kutty. "Robustness of Fairness: An Experimental Analysis." In Machine Learning and Principles and Practice of Knowledge Discovery in Databases: International Workshops of ECML PKDD 2021, Virtual Event, September 13-17, 2021, Proceedings, Part I, pp. 591-606. Cham: Springer International Publishing, 2022.

[15] Zhang, Yiliang, and Qi Long. "Assessing fairness in the presence of missing data." Advances in neural information processing systems 34 (2021): 16007-16019.

[16] Scutari, Marco, Francesca Panero, and Manuel Proissl. "Achieving fairness with a simple ridge penalty." Statistics and Computing 32, no. 5 (2022): 77.



``The properties of SDA estimator for constrained DI is studied in Section 4.1 while the properties of vanilla SGD with averaging is studied for the constrained DM problem in Section 4.2. I'm a bit confused about Section 4.2. Isn't this already covered in Fang et al 2018?"

This has been covered much before Fang et al 2018 in Polyak and Juditsky 1992 as we have stated after Theorem 4.2. Since the goal of our paper is to perform uncertainty quantification for fairness, and not proving a CLT for SGD iterates, we included this result for completion as Disparate Mistreatment is one of the most widely used fairness measures. 

``I was confused by the notation in Section 4.1. are the sensitive attributes in the training data . However are also referred to as the sequence of updates which is a weighted sum of all noisy gradients up to time . Have you perhaps double-loaded the notation for ?"

We have indeed double-loaded the notation. We will fix it in the final version. 

``Shouldn't the convergence in distribution result in Thm 4.1 be in terms of rather than ?"

We have used $n$ instead of $k$ to denote that $\bar{\theta}_n$ is the final iterate of the algorithm. But we understand why it could be confusing. We will change the notation. 

``

It seems like SDA is used to solve the constrained DI problem (Eqn 5), but vanilla SGD with Polyak-Ruppert averageing is used to solve the penalized DM problem (Eqn 7). Hasn't Fang et al already provided the theoretical results for UQ of vanilla SGD with PR averaging? Your contribution is geared towards SDA if I understand correctly. Is it necessary to spend time in this paper on the latter challenge if it's already more-or-less solved using Fang's results?"

This is true and we have clearly stated it in lines 322-327 that we extend the results of Fang et. al. 2018 to the SDA setting. Also we have mentioned after Theorem 4.2 that the results follow from  Polyak \& Juditsky, 1992. The only reason we have included this section is that, our goal is to do uncertainty quantification for fairness. Disparate Mistreatment (DM) is one of the most widely used fairness metric. For the sake of completion, we presented these results which hold for the alternative modeling of DM we propose. We will try to emphasize it more that the main theoretical contribution of this paper is towards SDA.

Dear PC, Senior AC and AC, 

We have several concerns about the reviews which we have elaborated. 

In summary, 

a) we urge you to consider that irrespective of the scores, all the **reviewers acknowledge that this is the first work** on Uncertainty Quantification (UQ) of fairness where we propose **a practically implementable algorithm with theoretical guarantee and illustrate its results on state-of-the-art classifiers and benchmark datasets**. 

b) We feel the scores are unfair since the reviewers consider **Theorem 5.1 as groundbreaking (Reviewer DCkP) and that it can stand on its own (Reviewer E7Th), but recommend "Reject" due to grammatical errors (Reviewer DCkP), misunderstanding of the results (Reviewer fp72), or because they felt that benchmark datasets ( Reviewer Erji agrees with us) in online fairness classification literature are just ``toy" examples (Reviewer E7Th).**

We would appreciate if you could take this into consideration and at least ignore the review of Reviewer fp72 or find another expert reviewer to evaluate the contributions of our paper. Thanks a lot for your consideration.

Sincerely

Authors






**Detailed concerns**

1. It appears to us that Reviewer fp72 is truly unaware of stochastic optimization and distributional convergence. They correctly identify that Theorem 5.1 is the main theoretical contribution but by their own admission in Q1, Reviewer fp72 does not understand what Theorem 5.1 says (which is distributional convergence of bootstrap estimator).  

2. Reviewer fp72 claims (Q2) "Figure 1 shows that DI is unstable ... especially in the early stage" whereas Fig. 1 shows the exact opposite that towards the end stage, when the trajectory is stable, there can be significant variations due to the stochasticity of the algorithm.

3. Reviewer fp72 claims that (Q3) ``can do a bootstrap method on testing set using trained model to get a confidence interval" which completely misses the fact that the trained model itself is random and the bootstrap method is designed to capture that.

4. Reviewer fp72 claims (Q4) that the stochasticity of the algorithm does not capture the effect of training distribution whereas the only source of randomness of the training algorithm is indeed the training data distribution and our results do capture that through the asymptotic covariance term.

5. The main criticism of Reviewer DCkP is that the paper has grammatical issues. 

6. Reviewer E7Th claims that state-of-the-art datasets used in online fairness-aware classification literature are toy examples and not organically online. Please find supporting citations in our reply to Reviewer E7Th.

Second reply to Reviewer E7Th.

"If we wanted to understand the variability in the fairness metric (DI/DM) arising from the stochasticity of the training dynamics, we simply need to repeat the training many times and record the resulting DI from each repetition. This seems more straightforward and vastly preferable to the proposed bootstrap procedure. ...."

We respectfully disagree on two accounts. 

a) Repeating the whole training many times with different training data **directly contradicts with online** training regime. In fact, the **main challenge** of online training is that the learner has access to **only one data point at every time step**, that is the we are **constructing the confidence interval** from a **single trajectory of data samples.**

b) Even if one relaxes online requirement, this approach still increases the data burden /sample complexity of the algorithms. 

We request you to kindly have a look at the inference results in online stochastic approximation literature [1-3] below. 

My bigger concern is ... For UQ to be useful in the setting you consider, we must understand how (classification loss, DI/DM) varies jointly in the accuracy-fairness space. It is not meaningful to consider only the fairness variability when the classification loss is also subject to the same forces of variability.

Note that our method and results characterize and estimate the uncertainty of the *model parameter* of a fairness-aware classification model. Since accuracy and fairness both depend on the same model parameter, using the same methods as in Algorithm 2 and Theorem 5.1, it is straightforward to get a similar result for accuracy as well. Indeed one can establish similar inference results for loss of a classifier as well. Since UQ of the fairness is the main gap in the research we are addressing here, we decided against providing a version of Theorem 5.1 for all possible properties of the classifier. In other words, **instead of looking at the joint distribution of accuracy/loss and fairness, we construct the confidence interval for the marginal distribution of fairness once the accuracy has stabilized. This is analogous to inference results for Gaussian mean estimation where the confidence intervals are constructed for the mean and not for other properties of the distribution, e.g., higher-order moments, skewness, kurtosis etc, even though the mean parameter of the Gaussian distribution controls all the properties of the distribution.**

[1] Polyak, Boris T., and Anatoli B. Juditsky. "Acceleration of stochastic approximation by averaging." SIAM journal on control and optimization 30, no. 4 (1992): 838-855.

[2] Duchi, John, and Feng Ruan. "Asymptotic optimality in stochastic optimization." arXiv preprint arXiv:1612.05612 (2016).

[3] Yixin Fang, Jinfeng Xu, and Lei Yang. Online bootstrap confidence intervals for the stochastic
gradient descent estimator. The Journal of Machine Learning Research, 19(1):3053–3073, 2018.



Dear AC, Senior AC, and PC, 

From response in the discussion period, it seems Reviewer E7Th is hostile and lacks understanding of the problem setting.

The first comment, "...we simply need to repeat the training many times..." clearly shows that Reviewer E7Th does not have the basic understanding of the online learning and stochastic approximation literature since the **main challenge** of inference of online stochastic approximation is to construct CI from a **single trajectory of data sequence with access to only one data point at each time point.** 

In the second comment, Reviewer E7Th claims that CI for fairness is meaningless without CI for loss/accuracy of the classifier since both depend on the variability in the model parameter. By this argument, for any inference to be meaningful, one needs to construct simultaneous CI for all possible properties of the model since all these properties depend on the variability of the estimated model parameter which is an absurd claim. For analogy, in Gaussian mean estimation, the confidence intervals are constructed for the mean and not for other properties of the distribution, e.g., higher-order moments, skewness, kurtosis etc, even though the mean parameter of the Gaussian distribution controls all the properties of the distribution.

We emphasize that our method and results characterize and estimate the uncertainty of the **model parameter of a fairness-aware classification model** and provide UQ of fairness when the training accuracy has reached a stable level. Since **UQ of the fairness is the main gap** in the research we are addressing here, we decided against providing a version of Theorem 5.1 for loss/accuracy of the classifier.  

We expect a fair review and request you to interfere. 

With regards,

Authors

Dear AC, Senior AC, and PC, 

 We draw your attention to the fact that **Reviewer fp72 has acknowledged that they initially misunderstood the paper and now has adjusted the score to 6.** This further strengthens our claim that **Reviewer E7Th is either hostile or has misunderstood the paper since they say their "initial hesitation towards this work is summed up by Reviewer fp72's Question 3".**

Furthermore, **Reviewer DCkP** has not got back to us with any further question. Reviewer DCkP's main criticism is that the paper has **grammatical/writing issues which is easily fixable.** We will do a thorough correction of these mistakes in the final version.

We request you to kindly take these into consideration.


With regards,
Authors


